Guiding the Guidance: A Comparative Analysis of User Guidance Signals for Interactive Segmentation of Volumetric Images

Interactive segmentation reduces the annotation time of medical images and allows annotators to iteratively refine labels with corrective interactions, such as clicks. While existing interactive models transform clicks into user guidance signals, which are combined with images to form (image, guidance) pairs, the question of how to best represent the guidance has not been fully explored. To address this, we conduct a comparative study of existing guidance signals by training interactive models with different signals and parameter settings to identify crucial parameters for the model's design. Based on our findings, we design a guidance signal that retains the benefits of other signals while addressing their limitations. We propose an adaptive Gaussian heatmaps guidance signal that utilizes the geodesic distance transform to dynamically adapt the radius of each heatmap when encoding clicks. We conduct our study on the MSD Spleen and the AutoPET datasets to explore the segmentation of both anatomy (spleen) and pathology (tumor lesions). Our results show that choosing the guidance signal is crucial for interactive segmentation as we improve the performance by 14% Dice with our adaptive heatmaps on the challenging AutoPET dataset when compared to non-interactive models. This brings interactive models one step closer to deployment on clinical workflows. We will make our code publically available.

==> sections/misc/input_adapter_line_plot.tex <==
\begin{figure}[]\ContinuedFloat
     \centering
     
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/input_adapter/enc_epoch=100_msd.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{-0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/input_adapter/enc_epoch=100_autopet.pdf}     
     \end{subfigure}
    %\caption{Influence of the input adapter (enc) on the performance on MSD Spleen~\cite{MSD-Spleen} (left) and AutoPET~\cite{autopet} (right).}
    %\label{fig:input_adaptor}
\end{figure}


==> sections/misc/interaction_probability_line_plot.tex <==
\begin{figure}[]
     \centering
     
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/interaction_probability/p_epoch=100_msd.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{-0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/interaction_probability/p_epoch=100_autopet.pdf}     
     \end{subfigure}
    \caption{Influence of the input adapter (top row) and the interaction probability $p$ parameter (bottom row) on the performance on the MSD Spleen~\cite{MSD-Spleen} (left) and on the AutoPET~\cite{autopet} dataset (right).}
    \label{fig:interaction_probability}
\end{figure}


==> sections/misc/sigma.tex <==
\begin{figure}[t]
     \centering
     
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{0.5cm}        

         \includegraphics[width=1.0\linewidth]{figures/sigma/boxplot_epoch=best_val_epoch_sigma_it=9_msd.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.45\linewidth}
        \hspace*{-0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/sigma/boxplot_epoch=best_val_epoch_sigma_it=9_autopet.pdf}
     \end{subfigure}
    \vspace*{-0.5cm}
    \caption{Influence of  $\sigma$ on the performance on MSD Spleen~\cite{MSD-Spleen} (left) and AutoPET~\cite{autopet} (right). The results are aggregated for all 5 guidance signals.}
    \label{fig:sigma_boxbplot}
\end{figure}


==> sections/misc/sigma_line_plot_autopet.tex <==
\begin{figure*}[h]
     \centering
     
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/disks_sigma_epoch=100_autopet.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/heatmaps_sigma_epoch=100_autopet.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/edt_sigma_epoch=100_autopet.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/gdt_sigma_epoch=100_autopet.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/exp_geos_sigma_epoch=100_autopet.pdf}         
     \end{subfigure}
    \caption{Dice improvement with multiple interactions for different $\sigma$ parameters on the MSD Spleen~\cite{MSD-Spleen} (first row) and the AutoPET~\cite{autopet} (second row) datasets.}
    \label{fig:sigma_line_plots}
\end{figure*}


==> sections/misc/sigma_line_plot_msd.tex <==
\begin{figure*}[h]\ContinuedFloat
     \centering
     
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/disks_sigma_epoch=100_msd.pdf}         
     \end{subfigure}
     %\hfill
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/heatmaps_sigma_epoch=100_msd.pdf}         
     \end{subfigure}
     %\hfill
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/edt_sigma_epoch=100_msd.pdf}         
     \end{subfigure}
     %\hfill
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/gdt_sigma_epoch=100_msd.pdf}         
     \end{subfigure}
     %\hfill
     \begin{subfigure}{0.18\linewidth}
         \includegraphics[width=1.0\linewidth]{figures/sigma/line_plots/exp_geos_sigma_epoch=100_msd.pdf}         
     \end{subfigure}

\end{figure*}


==> sections/misc/theta.tex <==
\begin{figure}[b]
     \centering
     
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{0.5cm}        

         \includegraphics[width=1.0\linewidth]{figures/theta/boxplot_epoch=best_val_epoch_theta_it=9_msd.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.45\linewidth}
        \hspace*{-0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/theta/boxplot_epoch=best_val_epoch_theta_it=9_autopet.pdf}
     \end{subfigure}
    \caption{Influence of the $\theta$ parameter on the performance on the MSD Spleen~\cite{MSD-Spleen} (left) and  AutoPET~\cite{autopet} dataset (right). The results are aggregated for the EDT and GDT guidances .}
    \label{fig:theta_boxplot}
\end{figure}

==> sections/misc/theta_line_plot_autopet.tex <==
\begin{figure}[]
     \centering
     
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/theta/line_plots/edt_theta_epoch=100_autopet.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{-0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/theta/line_plots/gdt_theta_epoch=100_autopet.pdf}         
     \end{subfigure}
    \caption{Dice improvement with multiple interactions for different $\theta$ parameters on the MSD Spleen~\cite{MSD-Spleen} (first row) and the AutoPET~\cite{autopet} (second row) datasets.}
    \label{fig:line_plots_theta}
\end{figure}


==> sections/misc/theta_line_plot_msd.tex <==
\begin{figure}[]\ContinuedFloat
     \centering
     
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/theta/line_plots/edt_theta_epoch=100_msd.pdf}         
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.45\linewidth}
     \centering        \hspace*{-0.5cm}        
         \includegraphics[width=1.0\linewidth]{figures/theta/line_plots/gdt_theta_epoch=100_msd.pdf}         
     \end{subfigure}
    % \caption{TODO}

\end{figure}


==> sections/text/sigma_results.tex <==
\iffalse
The final dice scores for different $\sigma$ values are presented in Fig. \ref{fig:results}a). The results on MSD Spleen~\cite{MSD-Spleen} show the highest dice scores at $\sigma=5$, with a slight improvement for two samples at $\sigma=1$, but performance decreases for higher values $\sigma>5$. Similarly, on AutoPET~\cite{autopet}, $\sigma=5$ and two samples with $\sigma=0$ show the best performance, while higher values demonstrate a significant performance drop. Differences between the results for different $\sigma$ values are more pronounced in AutoPET~\cite{autopet} as it is a more challenging dataset~\cite{AutoPET-Submission-1}, \cite{AutoPET-Submission-2}, \cite{AutoPET-Winner}.

Fig. \ref{fig:results}b) shows how the performance improves with new clicks for different $\sigma$. The best final and initial dice for disks and heatmaps are with $\sigma=1$ and $\sigma=0$. The difference is even more pronounced on AutoPET~\cite{autopet}. The same holds for the Euclidean maps, however, they stagnate for $\sigma=0$. Both Geodesic maps, on the other hand, exhibit lower Dice scores for small $\sigma < 5$ and achieve the best performance for $\sigma=5$ on both datasets. Another observation, which holds for all guidance signals, is that using larger $\sigma$ values leads to a worse initial Dice, which means that the models are more dependent on the guidance to perform well.
\fi
